Large Language Model Supply Chain: A Research Agenda

The rapid advancement of large language models (LLMs) has revolutionized artificial intelligence, introducing unprecedented capabilities in natural language processing and multimodal content generation. However, the increasing complexity and scale of these models have given rise to a multifaceted supply chain that presents unique challenges across infrastructure, foundation models, and downstream applications. This paper provides the first comprehensive research agenda of the LLM supply chain, offering a structured approach to identify critical challenges and opportunities through the dual lenses of software engineering (SE) and security & privacy (S\&P). We begin by establishing a clear definition of the LLM supply chain, encompassing its components and dependencies. We then analyze each layer of the supply chain, presenting a vision for robust and secure LLM development, reviewing the current state of practices and technologies, and identifying key challenges and research opportunities. This work aims to bridge the existing research gap in systematically understanding the multifaceted issues within the LLM supply chain, offering valuable insights to guide future efforts in this rapidly evolving domain.

==> chapters/7.related.tex <==
\section{Related Works}
In recent years, the LLM supply chain has garnered increasing attention from both academia and industry~\cite{jiang2022empirical,balayn2024empiricalexplorationtrustdynamics,balayn2024understandingstakeholdersperceptionsneeds}. Following our initial proposal of the concept of LLM supply chain, several subsequent works~\cite{hu2024llmsupplychain,huang2024llmsupplychain} have further expounded on and categorized different aspects of the LLM supply chain.
Huang et al.~\cite{huang2024llmsupplychain} provided a comprehensive overview of the LLM supply chain, detailing the stakeholders, composing artifacts, and supply types involved. They developed taxonomies of risk types, risky actions, and mitigations related to various supply chain stakeholders and components. Their work explores the technical and operational aspects of the LLM supply chain, offering valuable insights for researchers and practitioners.
Hu et al.~\cite{hu2024llmsupplychain} took a security-centric perspective on the LLM supply chain. They identified 12 potential security risks spanning different components and integration points of the LLM supply chain. Their work highlights the importance of security assurance across the entire LLM supply chain lifecycle, rather than just focusing on the model level.

Beyond these holistic studies of the LLM supply chain, other researchers have investigated specific aspects and subcomponents~\cite{jiang2023empirical,jiang2023ptmtorrent,montes2023discrepanciespretraineddeepneural,ajibode2024semanticversioningopenpretrained,wu2024new}. For example, Zhu et al.~\cite{zhu2025tensorapi} analyzed security risks associated with TensorFlow APIs that could enable transforming AI models into malware, such as file leaks, code execution, and shell access attacks. Zhao et al.~\cite{zhao2024models} conducted the first systematic study of malicious code poisoning attacks on pre-trained model hubs like Hugging Face, developing MalHug to detect and classify such threats. Chen et al.~\cite{liu2023demystifying} investigated remote code execution (RCE) vulnerabilities in LLM-integrated apps and frameworks, allowing prompt injection attacks, and proposed mitigation strategies. These works highlight the diverse security implications spanning the LLM supply chain, from model hubs and training pipelines to deployed applications integrated with LLMs.
While prior work has made important strides, the field of LLM supply chain research is still rapidly evolving with many open challenges remaining. 
